Computationally-efficient initialisation of GPs: The generalised variogram method

We present a computationally-efficient strategy to initialise the hyperparameters of a Gaussian process (GP) avoiding the computation of the likelihood function. Our strategy can be used as a pretraining stage to find initial conditions for maximum-likelihood (ML) training, or as a standalone method to compute hyperparameters values to be plugged in directly into the GP model. Motivated by the fact that training a GP via ML is equivalent (on average) to minimising the KL-divergence between the true and learnt model, we set to explore different metrics/divergences among GPs that are computationally inexpensive and provide hyperparameter values that are close to those found via ML. In practice, we identify the GP hyperparameters by projecting the empirical covariance or (Fourier) power spectrum onto a parametric family, thus proposing and studying various measures of discrepancy operating on the temporal and frequency domains. Our contribution extends the variogram method developed by the geostatistics literature and, accordingly, it is referred to as the generalised variogram method (GVM). In addition to the theoretical presentation of GVM, we provide experimental validation in terms of accuracy, consistency with ML and computational complexity for different kernels using synthetic and real-world data.

==> sections/contributions.tex <==
%!TEX root = ../tobar_cazelles_dewolff_TMLR2022.tex

\section{A likelihood-free covariance-matching strategy for training GPs}

Let us consider the zero-mean stationary process $y\sim\GP(0,K_{\theta})$ with covariance $K_{\theta}$ and hyperparameter $\theta\in\Theta$. Recall that the following statistic is an estimator of $K_\theta$.

\begin{definition}
\label{def:sample_cov}
Let $y\in\R$ be a zero mean stochastic process over $\R$ with observations $\vy = [y_1,\ldots,y_n]\in\R^n $ at times $\vt = [t_1,\ldots,t_n]\in\R^n$. The empirical covariance of $y$ is given by 
\begin{equation}
\label{eq:empirical_cov}
 \hat{K}_n(t) =  \sum_{i,j=1}^n \frac{y_iy_j\mathbf{1}_{t =t_i-t_j}}{\text{Card}\{t|t =t_i-t_j\}}.
\end{equation}
\end{definition}

We aim to find the hyperparameters of $y$ by projecting $\hat{K}_n(t)$ onto the parametrised family $\gK=\{K_\theta | \theta\in\Theta\}$. That is, by finding $\theta^*$ such that  $K_\theta(\cdot)$ is \emph{as close as possible} to $\hat{K}_n(t)$ in \eqref{eq:empirical_cov}, i.e., 
\begin{equation}
  \theta^*_n = \argmin_{\theta \in \Theta} D(\hat{K}_n, K_{\theta}),\label{eq:empirical_loss}
\end{equation}
where the function $D(\cdot,\cdot)$ is the chosen criterion for similarity. \CR{The proposed method builds on two types of (covariance) similarity. First, those operating directly on $\hat{K}_n$ and $K_{\theta}$, known as \textbf{temporal} divergences, which include the $L_1$ and $L_2$ distances. Second, those operating over the Fourier transforms of $\hat{K}_n$ and $K_{\theta}$, known as \textbf{spectral} divergences which are presented as follows.}


\subsection{Fourier-based covariance divergences}

If the covariance  $K_\theta$ is integrable and stationary, Bochner's Theorem~\citep{bochner1959lectures} states that $K_\theta$ and the process' power spectral density (PSD), denoted $S_\theta$, are \emph{Fourier pairs}, that is,
\begin{equation}
\label{eq:fourier_pair}
%  S(\xi) =  \fourier{K} \defeq \int_\R K(t) e^{-j2\pi \xi t}d t \quad\& \quad    K(t) =  \afourier{S} \defeq \int_\R S(\xi) e^{j2\pi \xi t}d \xi.
 S_\theta(\xi) =  \fourier{K_\theta} \defeq \int_\R K_\theta(t) e^{-j2\pi \xi t}d t,
\end{equation}  
where $j$ is the imaginary unit and $\fourier{\cdot}$ denotes the Fourier transform. 

\begin{remark}
Since zero-mean stationary GPs are uniquely determined by their PSDs, any distance defined on the space of PSDs can be ``lifted'' to the space covariances and then to that of GPs.
\end{remark}

Similarly to the procedure of learning the hyperparameters of the GP by matching the covariance as in \eqref{eq:empirical_loss}, we can learn the hyperparameters by projecting now an estimator of the PSD, denoted $\hat S_n$, onto a parametric family  $\gS = \{S_{\theta}, \theta\in\Theta\}$, that is, 
\begin{equation}
  \theta^*_n = \argmin_{\theta \in \Theta} D_F(\hat S_n, S_{\theta}),\label{eq:D-GP}
\end{equation}
where $D_F(\cdot,\cdot)$ is a divergence operating on the space of PSDs. However, since the map $K_\theta\rightarrow S_\theta$ is one-to-one, \eqref{eq:empirical_loss} and \eqref{eq:D-GP} are equivalent when $D_F(\cdot,\cdot) = D(\fourier{\cdot},\fourier{\cdot})$ and $\gS = \fourier{\gK}$. 

We will consider parametric families $\gS$ with explicit inverse Fourier transform,  since this way $\theta$ parametrises both the kernel and the PSD and can be learnt in either domain. These families include the Dirac delta, Cosine, Square Exponential (SE), Student's $t$, Sinc, Rectangle, and their mixtures; \CR{see Figure \ref{fig:kernels_psds} in Appendix \ref{appendix:fourier} for an illustration of some of these PSDs and their associated kernels. }

\CR{
\begin{remark}[Recovering kernel parameters from PSD parameters] For a parametric Fourier pair ($K$, $S$), the Fourier transform induces a map between the kernel parameter space and the PSD parameter space. For the chosen kernel/PSD families, this map is bijective, which allows us to compute the estimated kernel parameters from the estimated PSD parameters (and vice versa); see Table \ref{tab:loc-scale} for two examples of parametric kernels and PSDs. Furthermore, based on this bijection we refer as $\theta$ to both kernel and PSD parameters.
\end{remark}
}

\subsection{A particular case with explicit solution}
\label{sec:exact-case}
Of particular relevance to our work is the $2$-Wasserstein distance ($W_2$) and \emph{location-scale} families of PSDs. 

\begin{definition}[Location–scale] 
\label{def:loc_scale}
A family of one-dimensional integrable PSDs is said to be of location-scale type if it is given by  
\begin{equation}
  \left\{S_{\mu,\sigma}(\xi) = \frac{1}{\sigma} S_{0,1} \left(\frac{\xi-\mu}{\sigma}\right), \mu\in\R,\sigma\in\R_+\right\},
\end{equation}
where $\mu\in\R$ is the location parameter, $\sigma\in\R_+$ is the scale parameter and $S_{0,1}$ is the prototype of the family. 
\end{definition}

For arbitrary prototypes $S_{0,1}$, location-scale families of PSDs are commonly found in the GP literature. For instance, the SE, Dirac delta, Student's $t$, Rectangular and Sinc PSDs, correspond to the Exp-cos, Cosine, Laplace, Sinc, and Rectangular kernels respectively. Location-scale families do not, however, include kernel mixtures, which are also relevant in our setting and will be dealt with separately. Though the prototype $S_{0,1}$ might also be parametrised (e.g., with a \emph{shape} parameter), we consider those parameters to be fixed and only focus on $(\mu,\sigma)$ for the rest of this section. \CR{ Table \ref{tab:loc-scale} shows the two families of location-scale PSDs (and their respective kernels) that will be used throughout our work.}
\begin{table}[t]
\small
\caption{Location-scale PSDs (left) and their covariance kernel (right) used in this work. We have denoted by $t$ and $\xi$ the time and frequency variables respectively.}
\label{tab:loc-scale}
\vspace{1em}
\centering
\begin{tabular}{l | c | c || l | c | c}
 \textbf{PSD} & $S_{\mu,\sigma}(\xi)$ & Prototype $S_{0,1}(\xi)$ & \textbf{Kernel} & $K_{\mu,\sigma}(t)$ &  $K_{0,1}(t)$ 
\\ \hline

Square-exp & $\exp\left(-\left(\frac{\xi-\mu}{\sigma}\right)^2\right)$ & $\exp(-\xi^2)$ & Exp-cos & $\sqrt{\pi}\sigma\exp(-\sigma^2\pi^2t^2)\cos(2\pi\mu t)$ & $\sqrt{\pi}\exp(-\pi^2t^2)$ 
\\ \hline
Rectangular & $\text{rect}\left(\frac{\xi-\mu}{\sigma}\right)$ &  $\text{rect}(\xi)$ & Sinc & $\sigma\text{sinc}(\sigma t)\cos(2\pi\mu t)$ & $\text{sinc}(t)$ 
%\\
%Rectangular & $\text{rect}(\omega_0t)$ & Sinc & $\frac{1}{\xi}\sin(\frac{\xi}{\omega_0})$
\end{tabular}
\end{table}



\begin{remark} 
\label{rem:loc-scale}
Let us consider a location-scale family of distributions with prototype $S_{0,1}$ and an arbitrary member $S_{\mu,\sigma}$. Their quantile (i.e., inverse cumulative) functions, denoted $Q_{0,1}$ and  $Q_{\mu,\sigma}$ respectively, obey
\begin{equation}
  Q_{\mu,\sigma}(p) = \mu + \sigma Q_{0,1}(p)\label{eq:loc-scale-Q}.
\end{equation} 
\end{remark}

The linear expression in \eqref{eq:loc-scale-Q} is pertinent in our setting and motivates the choice of the $2$-Wasserstein distance $W_2$. This is because for one-dimensional distributions, $W_2^2(S,S_\theta)$ can be expressed in terms of the quantile functions of $S$ and $S_\theta$, denoted respectively $Q$ and $Q_\theta$, given by 
\begin{align}
  W_2^2(S, S_{\theta}) &= \int_0^1 (Q_{\theta}(p) - Q(p))^2 d p.
\end{align}
We are now in position to state the first main contribution of our work.

\begin{theorem} 
\label{thm:convexWF}
If $\gS$ is a  location-scale family with prototype $S_{0,1}$, the minimiser of $W_2(S, S_{\mu,\sigma})$ is unique  and given by 
\begin{equation}
  \mu^* = \int_0^1 Q(p)d p \qquad \mbox{and} \qquad
  \sigma^* = \frac{1}{\int_0^1 Q_{0,1}^2(p)d p}\int_0^1 Q(p) Q_{0,1}(p)d p, \label{eq:soln_mu_sigma}
\end{equation}
where $Q$ is the quantile function of $S$. The PSD $S$ does not need to be location-scale.
\end{theorem}

\begin{sketch} The proof follows from the fact that $W_2^2(S, S_{\mu,\sigma})$ is convex both on $\mu$ and $\sigma$, which is shown by noting that its Hessian is positive via Jensen's inequality. Then, the first order conditions give the solutions in \eqref{eq:soln_mu_sigma}. The details of the proof can be found in Appendix \ref{appendix:proofs}.
\end{sketch}



\begin{remark} 
  Although integrals of quantile functions are not usually available in closed-form, computing \eqref{eq:soln_mu_sigma} is straightforward. First, $Q_{0,1}(p)$ is known for a large class of prototypes including SE and rectangles. Second, $\mu^*  = \E_{\rx\sim S}[x]$ and $\int_0^1 Q_{0,1}^2(p)d p=\E_{\rx\sim S}[x^2]$, where $\rx$ is a random variable with PDF $S$. Third, both integrals are one-dimensional and supported on $[0,1]$, thus numerical integration is inexpensive and precise, specially when $S$ has compact support.
\end{remark} 


As pointed out by \citet{WF2021}, $W_2^2(S, S_{\theta})$ is in general non-convex, however, for the particular case of the location-scale family of PSDs, convexity holds. \CR{Since this family includes usual kernel choices in the GP literature, Theorem \ref{thm:convexWF} guarantees closed form solution for the optimisation problem in \eqref{eq:D-GP} and thus can be instrumental for learning GPs without computing (the expensive) likelihood function.
} 

\subsection{Learning from data}

Our objective is to learn the parameters $\theta$ of the kernel $K$ by matching empirical data-driven estimates of the kernel $\hat K_n$ (or the PSD  $\hat S_n$) with a parametric form. We achieve this using metrics in the temporal domain, i.e., solving \eqref{eq:empirical_loss}, or in the spectral domain, i.e., solving \eqref{eq:D-GP}. Learning the hyperparameters in this manner is possible provided that the statistics $\hat K_n$ and $\hat S_n$ converge to $K$ and $S$ respectively.  We next provide theoretical results on the convergence of the optimal minimiser $\theta_n^*$. The first result, Proposition \ref{prop:empirical_ls}, focuses on the particular case of the $2$-Wasserstein distance and location-scale families,  presented in Section \ref{sec:exact-case}. 

\begin{proposition}
\label{prop:empirical_ls} 
For $S_\theta$ in a location-scale family, $S$ the ground truth PSD and $D_F=W_2^2$, $\E D_F(S, \hat S_n)\to0$ implies that the empirical minimiser $\theta^*_n$ in \eqref{eq:D-GP} converges to the true minimiser $\theta^*=\argmin_{\theta \in \Theta} D_F(S, S_{\theta})$, meaning that $\E |\theta^*_n- \theta^*|\to 0$.
\end{proposition} 
\vspace{-0.4cm}\begin{sketch} First, in the location-scale family we have $\theta = (\mu,\sigma)$. Then, the solutions in Theorem \ref{thm:convexWF} allow us to compute upper bounds for $\vert \mu^*-\mu^*_n\vert$ and $\vert \sigma^*-\sigma^*_n\vert $ via Jensen's and Hölder's inequalities, both of which converge to zero as $\E W_2^2(S, \hat S_n)\to0$.  The details of the proof can be found in Appendix \ref{appendix:proofs}.
\end{sketch}

The second result, Proposition ~\ref{prop:empirical_gen}, deals with the more general setting of arbitrary parametric families, the  distances $L_1,L_2,W_1,W_2$ and either temporal and frequency based estimators. To cover both cases, we will denote  $\hat f_n$ to  refer to either $\hat K_n$ or $\hat S_n$.  Let us also consider the parametric function $f_\theta\in\gH:=\{f_\theta | \theta\in\Theta\}$ and the ground truth function $f$ which denotes either  the groud truth covariance or ground-truth PSD. 

\begin{proposition}
\label{prop:empirical_gen} 
For general parametric families $\gH$, the empirical solution $\theta^*_n$ converges a.s. to the true solution $\theta^*$ under the following sufficient and stronger conditions: (i) $D=W_r$ or $L_r, r=1,2$, (ii) $D(\hat f_{n}, f)\xrightarrow [n\to \infty]{a.s.} 0$; (iii) $\theta_n\xrightarrow[n\to \infty]{} \theta \iff D(f_{\theta_n}, f_\theta)\to 0$; and (iv) the parameter space  $\Theta$ is compact.
\end{proposition} 
\vspace{-0.4cm}\begin{proof}
This result follows as a particular case from Theorem 2.1 in \citet{bernton2019parameter}, where the authors study general $r$-Wasserstein distance estimators for parametric families of distributions for empirical measures, under the notion of $\Gamma$-convergence or, equivalently, epi-convergence. The proof for the $L_r, r=1,2$ case is similar to that of $W_r$.
\end{proof}

  
With the above results, implementation of GVM  only requires defining $\hat K_n$ and $\hat S_n$. In practice, we use \eqref{eq:empirical_cov} for $\hat K_n$ due to its  known convergence properties. For $\hat S_n$, the usual choice is the  Periodogram ($\Sper$)~\citep{schuster1900periodogram}. Though $\Sper$ is asymptotically unbiased ($\forall \xi, \E\Sper(\xi)\to S(\xi)$), it is inconsistent, i.e., its variance does not vanish when $n\to\infty$~\citep{stoica2005spectral}[Sec.~2.4.2], meaning that Props.~\ref{prop:empirical_ls} \& \ref{prop:empirical_gen} do not guarantee $\theta^*_n\to \theta^*$. Luckily, the variance of $\Sper(\xi)$ can be reduced via \emph{windowing} and the Welch/Bartlett techniques which produce (asymptotically) consistent and unbiased estimates of $S(\xi), \forall \xi$~\citep{stoica2005spectral}. %, meaning that $\Swel$ and $\Sbar$ converge pointwise in the mean square sense to the true PSD. Therefore, as we are interested on the practical use of spectral metrics for learning, both the data-driven approximation $\hat S_n$ and the candidate $S_\theta$ will be defined on a compact finite-resolution support, meaning that the mean square pointwise convergence translates to the mean convergence in the $L_r$,  $r$-Wasserstein, $r=1,2$, senses and thus Propositions \ref{prop:empirical_ls} and \ref{prop:empirical_gen} can be applied. 











%In practice, the ground truth PSD $S$ is unknown and the kernel is to be identified only from observations $\vy = [y_1,\ldots,y_n]\in\R^n $ at times $\t = [t_1,\ldots,t_n]\in\R^n $. Therefore, for a data-driven estimation of $S$, denoted $\hat S_n$, we address the minimisation of the empirical loss
%\begin{equation}
%  \theta^*_n = \argmin_{\theta \in \Theta} D(\hat S_n, S_{\theta}),\label{eq:empirical_loss}
%\end{equation}
%and its relationship to the \emph{true} minimisation problem in eq.~\eqref{eq:D-GP}. First, Prop.~\ref{prop:empirical_ls} focuses on the special case of the $2$-Wasserstein distance and the location-scale family, while Prop.~\ref{prop:empirical_gen} deals with arbitrary parametric families and the  distances $L_1,L_2,W_1,W_2$
%  in Table \ref{table:metrics}.
%\begin{proposition}
%\label{prop:empirical_ls} 
%For $S_\theta$ in a location-scale family and $D=W_2^2$, $\E W_2^2(S_\theta, \hat S_n)\to0$ implies that the empirical minimiser $\theta^*_n$ in eq.~\eqref{eq:empirical_loss} converges to the true minimiser $\theta^*$ in eq.~\eqref{eq:D-GP}, i.e., $\E |\theta^*_n- \theta^*|\to 0$.
%\end{proposition} 
%\begin{sketch} First, in the location-scale family we have $\theta = (\mu,\sigma)$. Then, the solutions in Theorem \ref{thm:convexWF} allow us to compute upper bounds for $\vert \mu^*-\mu^*_n\vert$ and $\vert \sigma^*-\sigma^*_n\vert $ via Jensen's and Hölder's inequalities, both of which converge to zero as $\E W_2^2(S, \hat S_n)\to0$. [Full proof in the Supp.~Mat.] 
%\end{sketch}
%%\begin{remark}
%%As the convergence of $\theta^*_n$ towards $\theta^*$ is controlled by the convergence of $W_2^2(S, \hat S_n)$, one can obtain stronger convergence for $\theta^*_n$ by imposing stronger convergence on $W_2^2(S, \hat S_n)$.
%%\end{remark}
%\begin{proposition}
%\label{prop:empirical_gen} 
%For general parametric families, the empirical solution $\theta^*_n$ converges a.s. to the true solution in $\theta^*$ under the following sufficient and stronger conditions: (i) $D=W_r$ or $L_r, r=1,2$, (ii) $D(\hat S_{n}, S)\xrightarrow [n\to \infty]{a.s.} 0$; (iii) $\theta_n\xrightarrow[n\to \infty]{} \theta$ implies $D(S_{\theta_n}, S_\theta)\to 0$; and (iv) the parameter space  $\Theta$ is compact.
%\end{proposition} 
%\begin{sketch}
%This result follows as a particular case from Theorem 2.1 in \cite{bernton2019parameter}, where the authors study general $r$-Wasserstein distance estimators for parametric families of distributions for empirical measures, under the notion of $\Gamma$-convergence or, equivalently, epi-convergence. The proof for the $L_r, r=1,2$ case is similar to that of $W_r$.
%\end{sketch}
%
%\CR{Como vamos a poner enfasis en $K$ y $S$ (y no solo en $S$) voy a sacar/disminuir el siguiente párrafo}
%
%With the above results, implementation of spectrum-based learning of GPs only requires building the data-driven estimator $\hat S_n$ that fulfils the above requirements. The \emph{de facto} approximation is the widely-used Periodogram, which we denote $\Sper$ and can be traced back to the work of \cite{schuster1900periodogram}. However, though $\Sper$ is asymptotically unbiased ($\forall \xi, \E\Sper(\xi)\to S(\xi)$), it is inconsistent, i.e., the variance of $\Sper(\xi)$ does not vanish when $n\to\infty$ \cite{stoica2005spectral}[Sec.~2.4.2]. As a consequence, the Periodogram does not fulfil the condition $W_2^2(S, \Sper)\to0$ and thus Propositions \ref{prop:empirical_ls} \& \ref{prop:empirical_gen} do not guarantee $\theta^*_n\to \theta^*$. Luckily, the variance of $\Sper(\xi)$ can be reduced via classical techniques such as the the Blackman-Tukey method (also referred to as \emph{windowing}) and the Welch/Bartlett techniques, denoted $\Swel$ and $\Sbar$, which divide the data into $M\in\N$ segments to then average the Periodograms of each segment thus reducing the variance according to $1/M$. The Welch/Bartlett methods produce (asymptotically) consistent and unbiased estimates of $S(\xi), \forall \xi$ \cite{stoica2005spectral}, meaning that $\Swel$ and $\Sbar$ converge pointwise in the mean square sense to the true PSD. Therefore, as we are interested on the practical use of spectral metrics for learning, both the data-driven approximation $\hat S_n$ and the candidate $S_\theta$ will be defined on a compact finite-resolution support, meaning that the mean square pointwise convergence translates to the mean convergence in the $L_r$,  $r$-Wasserstein, $r=1,2$, senses and thus Propositions \ref{prop:empirical_ls} and \ref{prop:empirical_gen} can be applied. 
%  if we assume that their supports are bounded these data-driven estimates also converge in the mean $2$-Wasserstein sense and thus Proposition \ref{prop:empirical_ls} can be applied. 

%Indeed, by \cite{villani2009optimal}[Theorem 6.13], the $2$-Wasserstein distance for measures supported on a bounded set is itself bounded by the $\L_2$ metric (using H\"older's inequality) and the dominated convergence theorem allows to conclude. This cover cases such as Gaussian, Laplace, rectangular, and sinc PSDs and their finite mixtures \CR{Elsa: bounded?}\CB{(i) Prop1 only works for location-scale family, therefore not for finite mixture. (ii) In order to have that $\E(\Swel,S)\to 0$ or  $\E(\Sbar,S)\to 0$ to apply Prop 1, we need bounded support. We can maybe put this comment after the following one which is "computed on a finite (frequency) grid". (iii) I don't know if we can have almost sure convergence of $\Swel$ and $\Sbar$, in order to be able to apply Prop2.}. Furthermore, the estimates $\hat S_n$ are always supported on a bounded set in practice since they are computed on a finite (frequency) grid.


%\begin{remark}
%In practice, we will compare (discrete) estimates $\hat S_n$ and (continuous) parametric PSDs $S_\theta$. We emphasise that the Wasserstein distance is well suited to this task as it measures horizontal displacement of mass rather than vertical point-wise discrepancy. This sets our approach apart from a large body of distances/divergences that have been applied to PSDs such as the Euclidean, KL, and Itakura-Saito ones, which are vertical and cannot compare PSDs defined on different supports.  
%\end{remark}




==> sections/experiments.tex <==
%!TEX root = ../tobar_cazelles_dewolff_TMLR2022.tex

\section{Experiments}
This section illustrates different aspects of the proposed GVM \CR{through the following experiments (E):
\begin{itemize}
    \setlength\itemsep{0em}
  \item[E1:] shows that GVM, unlike ML, is robust to different initialisation values and subsets of observations,
  \item[E2:] studies the sensibility of GVM to the calculation of $\hat S_n$ using Periodogram, Welch and Bartlett,
  \item[E3:] validates the linear computational complexity of GVM in comparison to the full and sparse GPs,
  \item[E4:] exhibits the results of learning a 20-component spectral mixture GP using GVM with different spectral metrics, 
  \item[E5:] assesses the ability of GVM to produce initial conditions which are then passed to an ML routine that learns a spectral mixture GP with 4, 8, 12 and 16 components,
  \item[E6:] presents a toy example where GVM is used to fit a GP with an isotropic SE kernel to multi-input (5-dimensional) data.   
\end{itemize}
}
 The benchmarks were implemented on MOGPTK~\citep{wolff2021mogptk}, and the Python codes (in Appendix \ref{appendix:code}) will be released to the public.



\subsection[]{E1: Stability with respect to initial conditions (spectral mixture  kernel, $L_2$, temporal)}

This experiment assessed the stability of GVM with respect to random initial conditions and different realisations. We considered a GP with a 2-component spectral mixture kernel $K(t) = \sum_{i=1}^2\sigma^2_i\exp(-\gamma_i \tau^2)\cos(2\pi\mu_i \tau) + \sigma_\text{noise}^2\delta_\tau$ with hyperparameters $\sigma_1=2$, $\gamma_1=10^{-4}$, $\mu_1=2\cdot10^{-2}$, $\sigma_2=2$,$\gamma_2=10^{-4}$, $\mu_2=3\cdot10^{-2}$, $\sigma_\text{noise}=1$. We produced 4000-point realisations from the GP and 50 random initial conditions $\{\theta^r\}_{r=1}^{50}$ according to $[\theta^r]_i\sim\text{Uniform}[\tfrac{1}{2}\theta_i,\tfrac{3}{2}\theta_i]$, where $\theta_i$ is the $i$-th true hyperparameter.

We considered two settings: i) train from $\{\theta^r\}_{r=1}^{50}$ using ML, and ii) compute GVM from $\{\theta^r\}_{r=1}^{50}$ and then perform ML. Each procedure was implemented using a single  realisation (to test stability wrt $\theta^r$) and different realisations (to test stability wrt the data). Our estimates $\hat\theta_i$ were assessed in terms of the  NLL and the relative mean absolute error (RMAE) of the parameters $\sum_{i=1}^8|\theta_i-\hat\theta_i|/|\theta_i|$.

Fig.~\ref{fig:stability} shows the NLL (left) and RMAE (right) versus computation time, for the cases of fixed (top) and different (bottom) observations; all times start from $t=1$ to use the logarithmic scale. First, in all cases the GVM initialisation (in red) took about half a second and resulted in an NLL/RMAE virtually identical to those achieved by ML initialised by GVM, this means that GVM provides reliable parameters and not just initial conditions for ML. Second, for the fixed observations (top), the GVM was stable wrt $\theta^r$ unlike ML which in some cases diverged. Third, for the multiple observations (bottom) GVM-initialised ML diverged in two (out of 50) runs, which is far fewer than the times that random-initialised ML diverged.



\begin{figure}[h]
  \includegraphics[width=0.49\textwidth]{img/exp1_NLL_fixed.pdf} \hfill
  \includegraphics[width=0.49\textwidth]{img/exp1_error_fixed.pdf}
  \includegraphics[width=0.49\textwidth]{img/exp1_NLL_free.pdf} \hfill
  \includegraphics[width=0.49\textwidth]{img/exp1_error_free.pdf}
  \caption{GVM as initialisation for ML starting form 50 random initial conditions: proposed GVM (red), standard ML (green) and ML starting from GVM (blue). The top plots consider a single dataset, while the bottom plots consider different realisations for each initial condition. The L-BFGS-B optimizer was used with the default gradient tolerance in order for the results to be comparable.}
  \label{fig:stability}
\end{figure}


\subsection[]{E2: Sensibility of GVM wrt the Periodogram (exact case: $W_2$, location-scale)}

We then considered kernels with location-scale PSDs and the $W_2$ metric over the PSDs. This case has a unique solution but requires us to compute $\hat S_n$ in \eqref{eq:D-GP}; this experiment evaluates different ways of doing so. We produced 4000 observations \textbf{evenly-sampled} in $[0,1000]$ from GPs with square exponential and rectangular PSDs (which correspond to the Exp-cos and Sinc kernels respectively---\CR{see Table \ref{tab:loc-scale}}), \CR{each with location $\mu \sim \text{U}[0.025,0.075]$ and scale $l \sim \text{U}[0.01,0.02]$}. We computed $\hat S$ via the Periodogram, Welch and Bartlett methods with different windows. \CR{Table \ref{tab:sensitivity} shows the percentage relative error (PRE)\footnote{PRE = $100\frac{|\theta-\hat\theta|}{\theta}$, where $\theta$ is the true parameter and $\hat\theta$ its estimate.} averaged over 50 runs}. \CR{The estimates of both parameters are fairly consistent: their magnitude does not change radically for different windows and Periodogram methods. In particular, the estimates of the location parameter are accurate with an average error in the order of 2\% for both kernels. The scale parameter was, however, more difficult to estimate, this can be attributed to the spectral energy spread in the Periodogram, which, when using the Wasserstein-2 metric, results in the scale parameter to be overestimated. }For both kernels and $\mu=0.05, l=0.01$, the case of the (windowless) Periodogram is shown in Fig.~\ref{fig:sensibility} and the remaining cases are all shown in Appendix \ref{appendix:E2}. In the light of these results, we considered the Periodogram (no window) for the remaining experiments.  


\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1}


\begin{table*}[t]
\centering
\caption{
\CR{Performance of GVM learning GPs with the Exp-cos and Sinc kernels under different sampling settings, Periodogram methods and windows. Each entry of the table shows the average percentage relative error for location (left) and scale (right), with their standard deviations, separated by the symbol "/". True parameters where $\mu \sim \text{U}[0.025,0.075]$ and $l \sim \text{U}[0.01,0.02]$; averages and standard deviations computed over 50 runs.}}
\label{tab:sensitivity}
\small
\begin{tabular}{cl|ccc}
\toprule
              Kernel      &   Window   & Periodogram           & Bartlett               & Welch                   \\ \hline
\multirow{3}{*}{Exp-cos}  & none & 2.30\p1.61/33.41\p13.27 & 2.17\p1.91/20.88\p11.69  & 2.05\p1.64/24.87\p14.35    \\
                          & hann & 2.98\p2.14/34.93\p14.33 & 3.02\p2.36/26.23\p13.05  & 2.52\p1.75/31.83\p13.29    \\
                          & hamming & 2.92\p2.04/34.93\p14.16 & 2.93\p2.29/27.35\p13.26  & 2.49\p1.73/32.26\p13.22  \\ \hline
\multirow{3}{*}{Sinc}     & none & 2.36\p1.65/8.93\p6.73 & 2.63\p2.23/83.23\p26.39 & 2.31\p1.77/38.87\p15.95   \\
                          & hann & 2.68\p2.02/10.03\p9.22 & 2.59\p1.77/58.86\p17.48  & 2.44\p1.78/19.52\p11.32    \\
                          & hamming & 2.60\p2.01/9.62\p8.93 & 2.56\p1.75/50.62\p15.79 & 2.43\p1.76/16.51\p10.75    \\ \bottomrule
\end{tabular}
\end{table*}



\begin{figure}[ht]
  \includegraphics[width=0.49\textwidth]{img/effect_SM_periodogram_None.pdf}
  \includegraphics[width=0.49\textwidth]{img/effect_sinc_periodogram_None.pdf}
  \caption{GVM estimates for Exp-cos (top) and Sinc (bottom) kernels shown in red against $\hat S$ (blue) and true kernels (black). This case: Periodogram, no window.}
  \label{fig:sensibility}
\end{figure}



\subsection{E3: Linear complexity (exact case)} 

%\begin{wrapfigure}{r}{0.55\textwidth}
%\centering
%  \includegraphics[width=0.55\textwidth]{img/exp2.pdf}
%  \caption{Training times vs number of datapoints.}
%  \label{fig:comp_cost}
%\end{wrapfigure}

We then evaluated the computation time for the exact case of GVM ($W_2$ distance and location-scale family) for an increasing amount of observations. We considered \textbf{unevenly-sampled} observations from an single component SM kernel ($\mu=0.05, \sigma=0.01$) in the range $[0,1000]$. We compared GVM against i) the ML estimate starting from the GVM value (full GP, 100 iterations), and ii) the sparse GP using 200 pseudo inputs~\citep{sparseGP}. Fig.~\ref{fig:comp_cost} shows the computing times versus the number of observations thus validating the claimed linear cost of GVM and its superiority wrt to the rest of the methods. The (solid line) interpolation in the plot is of linear order for GVM, linear for sparse GP since the number of inducing points is fixed, and cubic for the full GP. 

\begin{figure}[ht]
\centering
  \includegraphics[width=0.7\textwidth]{img/exp2.pdf}
  \caption{Training times vs number of datapoints for the proposed GVM, full GP and sparse GP.}
  \label{fig:comp_cost}
\end{figure}

%Additionally, Fig.~\ref{fig:comp_cost} (bottom) shows the estimated parameters for SL-GP and maximum likelihood. Notice that SL-GP succeeds in estimating both parameters for more that 750 observations and that ML benefits from SL-GP's initial conditions except for some instances around 500 iterations (for the location parameter). The fact that SL-GP fails to identify the parameters for fewer than 750 observations is explained from the fact that the 95\% of the model (Gaussian) spectral energy is concentrated on frequencies $[\mu-2\sigma,\mu+2\sigma] = [0.03,0.07]$, meaning that the (approximate) Nyquist frequency is $f_N = (2\pi*0.14)$ and is equivalent to sampling 879 observations in the considered range $[0,1000]$. This further validates the SL-GP estimates from a Nyquist \cite{Nyquist_1928,Shannon_1949} perspective.



\subsection[]{E4: Fitting a 20-component spectral mixture (different spectral metrics)}

This experiment shows the effect of different spectral distances in the GVM estimates using a real-world audio signal from the Free Spoken Digit Dataset\footnote{\url{https://github.com/Jakobovski/free-spoken-digit-dataset}}. We trained a 20-component SM kernel~\citep{pmlr-v28-wilson13}, a kernel known to be difficult to train, and considered the distances $L_1$, $L_2$, $W_1$ and $W_2$ (spectral); Itakura-Saito and KL were unstable and left our of the comparison. Fig.~\ref{fig:fitting_mixtures_audio} shows the results of the GVM: observe that under almost all metrics, the 20-component spectral mixture matches the Periodogram (\CR{considered to be the ground truth PSD in this case}). The exception is $W_2$ which struggles to replicate the PSD peaks due to its objective of averaging mass \emph{horizontally}. 

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.49\textwidth]{img/audio_L1.pdf}
    \includegraphics[width=0.49\textwidth]{img/audio_L2.pdf}
      \includegraphics[width=0.49\textwidth]{img/audio_W1.pdf}
        \includegraphics[width=0.49\textwidth]{img/audio_W2.pdf}
  \caption{GVM matching Periodogram with a 20-component SM under different spectral metrics.}
  \label{fig:fitting_mixtures_audio}
\end{figure}


\subsection[E5: Learning spectral mixtures and parameter initialisation (L2, multiple orders)]{E5: Learning spectral mixtures and parameter initialisation ($L_2$, multiple orders)}

\begin{figure}[ht]
\centering
  \includegraphics[width=0.24\textwidth]{img/losses_SM4.pdf}
  \includegraphics[width=0.24\textwidth]{img/losses_SM8.pdf}
  \includegraphics[width=0.24\textwidth]{img/losses_SM12.pdf}
  \includegraphics[width=0.24\textwidth]{img/losses_SM16.pdf}
  \caption{NLLs for the SE spectral mixtures (4,8,12 and 16 components) with different initialisation strategies.}
  \label{fig:losses_SM}
\end{figure}

In this experiment, GVM was implemented to find the initial conditions of a GP with SM kernel (4, 8, 12 and 16 components) to a real-world 1800-point heart-rate signal from the MIT-BIH database\footnote{\url{http://ecg.mit.edu/time-series/}}. We considered the $L_2$ metric (spectral) minimised with Powell and then passed the hyperparameters to an ML routine for 1500 iterations (using Adam with learning rate = 0.1). This methodology was compared against the random initialisation and provided by MOGPTK based on Bayesian nonparametric spectral estimation (BNSE)~\citep{tobar2018bayesian}. Fig.~\ref{fig:fitting_mixtures} first shows the GVM approximations to the heart-rate PSD using 16-component spectral mixtures, for both both kernels.


%\begin{wraptable}{r}{0.4\textwidth}
%\scriptsize
%\centering
%\caption{Computation times (secs) for fitting SMs.}
%\label{tab:init_SM}
%\begin{tabular}{lcccc}
%\toprule
%                    & 4-comp & 8-comp & 12-comp  & 16-comp \\ 
%\midrule
%GVM init & \textbf{2.6}          & \textbf{7.6}          & \textbf{10.9}  &  \textbf{23.9}       \\
%BNSE init & 74.6         & 68.9          & 72.0    &74.1      \\
%ML          & 420.3        & 464.6         & 529.2   & 582.6 \\       
%\bottomrule
%\end{tabular}
%\end{wraptable}

\begin{table}[h]

%\scriptsize
\centering
\small
\caption{Computation times (secs) for fitting SMs.}
\label{tab:init_SM}
\begin{tabular}{lcccc}
\toprule
                    & 4-comp & 8-comp & 12-comp  & 16-comp \\ 
\midrule
GVM init & \textbf{2.6}          & \textbf{7.6}          & \textbf{10.9}  &  \textbf{23.9}       \\
BNSE init & 74.6         & 68.9          & 72.0    &74.1      \\
ML          & 420.3        & 464.6         & 529.2   & 582.6 \\       
\bottomrule
\end{tabular}

\end{table}

Fig.~\ref{fig:losses_SM} shows NLL for the cases considered. Observe that: i) the non-initialised ML training becomes trapped in local minima in all four cases, ii) the initialisation provided by GVM provides a dramatic reduction of the NLL, even wrt to the BNSE initialisation, iii) the ``elbow'' at the beginning of the GVM-initialised case suggests that the ML training could have run for a a few iterations (e.g., 100) and still reach a sound solution. Table \ref{tab:init_SM} shows the execution times and reveals the superiority of GVM also in computational time. 

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.49\textwidth]{img/16-specM-HR.pdf}
  \includegraphics[width=0.49\textwidth]{img/16-sincM-HR.pdf}
  \caption{GVM approximations of the PSD of a 1800-sample heart-rate signal using 16-components SE (top) and rectangular (bottom) mixtures. Training time shown above each plot.}
  \label{fig:fitting_mixtures}
\end{figure}



\subsection[]{E6: Learning an isotropic SE kernel (standard variogram, 5-dimensional inputs, $L_2$)}
\label{sec:E6}

%\begin{wrapfigure}[12]{r}{0.55\textwidth}
%\centering
%  \includegraphics[trim={3.2cm 0 3.2cm 0},clip,width=0.55\textwidth]{img/exp6.pdf}
%  \caption{Empirical covariance and fitted covariance function. The data consisted of 1000 5-dimensional datapoints.}
%  \label{fig:isotropic}
%\end{wrapfigure}

\CR{Though our work focuses on the single-input-dimension case, recall that the GVM method is applicable to datasets of arbitrary input dimension, therefore, to motivate the use of GVM for multi-input GPs, we present a minimal multi-input example. We considered a 5-dimensional GP with SE kernel $K(\tau) = \sigma^2\exp(-\tfrac{1}{2l^2}||\tau||^2) + \sigma_\text{noise}^2\delta_t$, and considered four sets of values for the hyperparameters. Notice that though we consider 5-dimensional input data, we assume that all dimensions have the same scale parameter, this is the usual setting of the Variogram method in Geostatistics~\citep{cressie1993stats,chiles1999geo}. For each set of hyperparameters, we sampled 1000 points and then implemented GVM with the $L_2$ (temporal) distance to learn the GP. Table \ref{tab:multi-input} shows the estimate error and standard deviation for each hyperparameter, from which the applicability of GVM to address the isotropic multi-input case can be confirmed. }For illustration and resemblance to the standard variogram method, Fig.~\ref{fig:isotropic} shows the case $\sigma^2=5$, $l=1$, and $\sigma_\text{noise}=1$, where the learnt hyperparameters were $\hat\sigma^2=5.85$, $\hat l=1.09$, and $\hat\sigma_\text{noise}=1.02$.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.7\textwidth]{img/exp6.pdf}
  \caption{Empirical covariance and fitted covariance function via GVM. The data consisted of 1000 5-dimensional datapoints.}
  \label{fig:isotropic}
\end{figure}

\begin{table}
\centering
\small
\caption{\CR{GVM applied to multi-input data for four runs of synthetic data using different hyperparameters, i.e., $\sigma^2,l,\sigma_\text{noise}^2$. For each set of hyperparameter, $n=100$ runs were executed to calculate the mean and standard deviation of the estimates (i.e., $\hat{\sigma}^2,\hat{l},\hat{\sigma}_\text{noise}^2$).}}
\label{tab:multi-input}
\vspace{1em}
\begin{tabular}{c|ccc|ccc}
    \hline
    Run & $\sigma^2$ & $l$ & $\sigma_\text{noise}^2$ & $\hat{\sigma}^2$ & $\hat{l}$ & $\hat{\sigma}_\text{noise}^2$ \\
    \hline
    1 & 5 & 2 & 1 & 5.20 ± 2.07 & 0.50 ± 0.09 & 0.91 ± 0.68 \\
    2 & 15 & 2 & 2 & 14.12 ± 13.14 & 2.07 ± 1.09 & 2.04 ± 1.51 \\
    3 & 3 & 3 & 0.5 & 2.68 ± 3.33 & 3.24 ± 1.65 & 0.97 ± 0.71 \\
    4 & 0.5 & 5 & 0.5 & 0.45 ± 0.62 & 3.96 ± 2.50 & 0.56 ± 0.30 \\
    \hline
\end{tabular}
\end{table}






==> sections/practical.tex <==
%!TEX root = ../tobar_cazelles_dewolff_TMLR2022.tex


\section{Practical considerations}

\CR{
This section is dedicated to the implementation of GVM. We first present  Algorithms \ref{alg:temporal} and \ref{alg:spectral} to clearly illustrate the application of GVM using the temporal and spectral metrics respectively. Then, the following subsections discuss the general case (when the family of PSDs is not location scale), the computational complexity, the noise variance parameter and the relationship between GVM and ML solutions.}

\begin{minipage}{0.36\textwidth}
	\begin{algorithm}[H]
		\caption{GVM - Temporal loss}\label{alg:temporal}
		\begin{algorithmic}
			\Require $t_i,y_i, i=1,\ldots,n$
			\Require parametric family $\{K_\theta\}_{\theta\in\Theta}$
			\Require  {temporal} metric $D(\cdot,\cdot)$\\
			Compute $\hat K _n$ as in eq.~(\ref{eq:empirical_cov})\\
			Construct loss $\theta \mapsto D(K_\theta, \hat K_n)$\\
			Find $\theta_n^\star$ in eq.~(\ref{eq:empirical_loss}) numerically or via gradient-based methods
		\end{algorithmic}
	\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.6\textwidth}
	\begin{algorithm}[H]
		\caption{GVM - Spectral loss}\label{alg:spectral}
		\begin{algorithmic}
			\Require $t_i,y_i, i=1,\ldots,n$
			\Require parametric family $\{S_\theta\}_{\theta\in\Theta}$
			\Require  {spectral} metric $D_F(\cdot,\cdot)$\\
			Compute $\hat S_n$, e.g., via Periodogram or applying $\mathcal{F}\{\cdot\}$ to  eq.~(\ref{eq:empirical_cov})\\
			Construct loss $\theta \mapsto D_F(S_\theta, \hat S_n)$
			\If{($D_F \Is W_2$) $\And$ ($\{S_\theta\}_{\theta\in\Theta}$\Is location-scale)}

			exact case: $\theta_n^\star$ given by eq.~(\ref{eq:soln_mu_sigma})
			\Else

				find $\theta_n^\star$ in eq.~(\ref{eq:D-GP}) numerically or using gradients
			\EndIf
		\end{algorithmic}
	\end{algorithm}
\end{minipage}




\subsection{Solving the general case: beyond the location-scale family}

Recall that the proposed method has a closed-form solution (at least) when one considers PSDs in location-scale family and the $W_2$ distance over the spectral domain. However, in the general case the corresponding minimisation is not convex in $\theta$ and thus iterative/numerical optimisation is needed. In particular, for horizontal Fourier distances the derivative of the loss depends on the derivative of the quantile function $Q_{\theta}$ which might not even be known in closed form in general, specially for mixtures. However, in most cases the lags of the empirical covariance or the frequencies of the Periodogram belong to a compact space and thus numerical computations are precise and inexpensive. Therefore, approximate derivatives can be considered (e.g., in conjunction with BFGS) though in our experiments the derivative-free Powell method also provide satisfactory results. 

\subsection{Linear computational complexity}

First, for temporal divergences (operating on the covariance) we can modify the statistic in \eqref{eq:empirical_cov} using \emph{binning}, that is, by averaging values for which the lags are similar; this process is automatic in the case of evenly-sampled data and widely used in discrete-time signal processing. This allows to reducing the amount of summands in $\hat K_n$ from $\tfrac{n(n+1)}{2}$ to an order $n$ or even lower if the range of the data grows beyond the length of the correlations of interests.

Second, for the exact case of the spectral divergences in Sec.~\ref{sec:exact-case} the cost of the $2$-Wasserstein loss is given by calculating i) the Periodogram $\hat S_n$, ii) its corresponding quantile function, and iii) the integrals in \eqref{eq:soln_mu_sigma}. The Periodogram has a complexity $\gO(nk)$, where $n$ is the number of observations and $k$ the number of frequency bins; in the evenly-sampled case, one could set $k=n$ and apply the fast Fourier transform at a cost $\gO(n\log n)$. However, for applications where the number of datapoints greatly exceeds the required frequency resolution,  $k$ can be considered to be constant, which results in a cost $\gO(n)$. The quantile functions and their integrals also have a linear cost but only in the number of frequency bins $\gO(k)$ since they are frequency histograms, therefore, computing the solution has a linear cost in the data. Lastly, for the general case using numerical optimisation methods, we need to calculate $\hat S_n$ or its quantile---which are $\gO(n)$---only once, to then compute the chosen distance $D$, which is $\gO(k)$ for discrete measures defined on a $k$-point grid, as many times as the optimisation routine requires it. Therefore, for the general case the cost is $\gO(k)$ but with a constant that depends on the complexity of the parametric family $\{S_\theta, \theta\in\Theta\}$ and the optimiser of choice.

\subsection{Noise variance and relationship to maximum likelihood}
\label{sec:non-unitary}

Following the assumptions of the Fourier transform, the spectral divergences considered apply only to Lebesgue-integrable PSDs, which rules out the relevant case of white-noise-corrupted observations. This is because white noise, defined by a Dirac delta covariance, implies a PSD given by a constant, positive, infinite-support, \emph{spectral floor} that is  non-integrable. These cases can be addressed with temporal divergences, which are well suited (theoretically and in practice) to handle noise. 

The proposed hyperparameter-search method is intended both as a standalone likelihood-free GP learning technique and also as a initialisation approach to feed initial conditions to a maximum likelihood (ML) routine.  In this sense, we identify a relationship between the ML estimator $\hat{\theta}_{ML}$ and the proposed estimator $\theta^*$, obtained from \eqref{eq:D-GP}, for $D_F=L_2$. From \eqref{eq:fourier_pair} and Plancherel's theorem, we have  $\Vert S -S_{\theta}\Vert_{L_2} = \Vert K -K_{\theta}\Vert_{L_2}$. Then, by definition of the estimators and Lemma 2 in \citet{hoffman2020black}, we obtain the following inequality
\begin{equation}
\KL(\rmK_0||\rmK_{\hat{\theta}_{ML}})\leq \KL(\rmK_0||\rmK_{\theta^*})\noindent \leq \frac{1}{2} \Vert \rmK_0^{-1}\Vert_2  \Vert \rmK_{\theta^*}^{-1}\Vert_2 \Vert \rmK -\rmK_{\theta^*}\Vert_{F},\label{eq:ineq_ML}
\end{equation}
where $\Vert\cdot\Vert_{F}$ denotes the matrix Frobenius norm, \CR{$\KL(A||B)$ denotes the KL divergence between zero-mean multivariate normal distributions with covariances $A$ and $B$,} and recall that  $\rmK_0$ is the kernel of the ground truth GP. Denoting the ball centred at 0 with radius $M$ by $B(0,M)$, we present the following remark.

\begin{remark} 
The inequality in \eqref{eq:ineq_ML} states that if the proposed estimator $\theta^*$ is such that $\Vert S -S_{\theta^*}\Vert_{L_2}\in B(0,M)$, then $\KL(\rmK_0||\rmK_{\hat{\theta}_{ML}})\in B(0,\frac{1}{2} \Vert \rmK_0^{-1}\Vert_2  \Vert \rmK_{\theta^*}^{-1}\Vert_2M)$. Therefore, under the reasonable assumption that the function $\theta\mapsto\rmK_\theta$ only produces well-conditioned matrices, the factor $\Vert \rmK_0^{-1}\Vert_2  \Vert \rmK_{\theta^*}^{-1}\Vert_2$ is bounded and thus both balls have radius of the same order.
\end{remark}


==> sections/preliminaries.tex <==
%!TEX root = ../tobar_cazelles_dewolff_TMLR2022.tex


\section{Preliminaries}

\subsection{Motivation}
\label{sec:motivation}
Let us consider $y\sim\GP(0,\CB{K})$ and its realisation $\vy = [y_1,\ldots,y_n]\in\sR^n $ at times $\vt = [t_1,\ldots,t_n]\in\sR^n$. The kernel $\CB{K}$ is usually learnt by choosing a family $\{K_\theta\}_{\theta\in\Theta}$ and optimising  the log-likelihood 
\begin{equation}
\label{eq:log_likelihood}
  l(\theta) = -\frac{1}{2} \Tr{(\rmK_\theta^{-1} \vy \vy^\top) } - \frac{1}{2} \log |\rmK_\theta| - \frac{n}{2}\log 2\pi,
\end{equation}
 with respect to $\theta\in\Theta$, where we used the cyclic property of the trace, and defined $\rmK_\theta \defeq K_\theta(\vt)$ according to $[\rmK_\theta]_{ij} = K_\theta(t_i-t_j), i,j\in\{1,\ldots,n\}$. Since  $\E{\vy \vy^\top} = \CB{K}(\vt) \defeq \CB{\rmK}$, we note that
\begin{equation}
  \label{eq:El}
  \E {l(\theta)} = -\frac{1}{2} \Tr{(\rmK_\theta^{-1} \CB{\rmK} )} - \frac{1}{2} \log |\rmK_\theta|- \frac{n}{2}\log 2\pi.
\end{equation}
Observe that, up to terms independent of $\theta$, \eqref{eq:El} is equivalent to negative Kullback-Leibler divergence (NKL) between the multivariate normal distributions $\gN(0,\CB{\rmK})$ and $\gN(0,\rmK_\theta)$ given by
\begin{equation}
\label{eq:NKL}
  \NKL(\CB{\rmK}||\rmK_\theta) = -\frac{1}{2}\left(\Tr{\rmK_\theta^{-1}\CB{\rmK}} - n  + \log\frac{|\rmK_\theta|}{|\CB{\rmK}|} \right).
\end{equation}

This reveals that learning a GP by maximising $l(\theta)$ in \eqref{eq:log_likelihood} can be understood (in expectation) as minimising the KL between the $\vt$-marginalisations of the true process $\GP(0,\CB{K})$ and a candidate process $\GP(0,K_\theta)$. This motivates the following remark.


\begin{remark} 
Since maximum-likelihood  learning of GPs has a cubic computational cost but it is (on average) equivalent to minimising a KL divergence, what other divergences or distances, computationally cheaper than the likelihood, can be considered for learning GPs? 
\end{remark}


\subsection{Divergences over covariance functions}

We consider zero-mean stationary GPs. The zero-mean restriction can be easily lifted by detrending the data using a parametric model. The stationary requirement allows us to i) aggregate observations in time when computing the covariance, and ii) compare covariances in terms of their (Fourier) spectral content. Therefore, we consider two types of divergences over covariances: i) \textbf{temporal} ones, which operate directly to the covariances, and ii) \textbf{spectral} ones, which operate over the the Fourier transform of the covariances, i.e., the GP's power spectral density (PSD). \CR{As our work relies extensively on concepts of spectral analysis and signal processing, a brief introduction to the subject is included in Appendix \ref{appendix:fourier}.} 

Though we can use most metrics (e.g., $L_1$, $L_2$) on both domains, the advantage of the spectral perspective is that it admits density-specific divergences as it is customary in signal processing~\citep{basseville1989distance}. Bregman divergences, which include the Euclidean, KL and Itakura-Saito (IS)~\citep{itakura1968analysis}, are \emph{vertical} measures, i.e, they integrate the point-wise discrepancy between densities across their support. We also consider \emph{horizontal} spectral measures, based on the minimal-cost to \emph{transport} the mass from one distribution---across the support space---onto another. This concept, known as optimal transport (OT)~\citep{villani2009optimal}  has only recently been considered for comparing PSDs using, e.g., the $1$- and $2$-Wasserstein distances,  denoted $W_1$ and $W_2$~\citep{WF2021,henderson2019audio}. \CR{See Appendix \ref{appendix:def_dist} for definitions of vertical and horizontal divergences.}

%Alternatively, one can construct novel distances among PSDs building on resources from optimal transport (OT) \cite{villani2009optimal}, which has emerged as a sound metric to compare probability distributions in settings where the topology of the distribution's support plays a key role as shown by \cite{kolouri2017optimal, courty2016optimal, peyre2019computational}. Specifically, OT finds the minimal-cost procedure to \emph{transport} the mass from one distribution---across the support space---onto another one and thus are considered to be \emph{horizontal} distances. OT has only recently been considered for comparing PSDs using, e.g., the $1$- and $2$-Wasserstein distances,  denoted $W_1$ and $W_2$: \cite{WF2021} proposed the Wasserstein-Fourier (WF) distance as a general-purpose similarity function for time series and \cite{henderson2019audio} performed an interpolation of audio signals in the spectral domain, or \emph{portamento}, solving a OT problem between PSDs.  Table \ref{table:metrics} shows the spectral metrics considered in our work.

\iffalse
\begin{table}[t]
\caption{Divergences and their definitions. $S$ stands for the (power spectrum) density function and $Q$ for the quantile function.}
\small
\centering
\begin{tabular}{m{2.5cm} m{3.7cm} m{3.5cm} m{2.7cm}}
\toprule
Divergence  & Definition      \\ 
\midrule
$L_1$             & $\int_\sR|S(\xi)-S'(\xi)|d\xi$   \\\hline
$L_2$             & $\int_\sR(S(\xi)-S'(\xi))^2d\xi$ \\\hline
$W_1$  &  $\int_0^1 | Q(p)-Q'(p)|d p$     \\\hline
$W_2$ &   $\int_0^1(Q(p)-Q'(p))^2d p$     \\\hline
Kullback-Leibler  &     $\int_\sR \log\left(\frac{S(\xi)}{S'(\xi)}\right) S(\xi)d\xi$   \\\hline
Itakura-Saito     &  $\int_\sR\left(\frac{S(\xi)}{S'(\xi)}-\log\frac{S(\xi)}{S'(\xi)}-1\right)d\xi$      \\\bottomrule
\end{tabular}
\label{table:metrics}
\end{table}

\fi
\iffalse
%% old  and more complete table
\begin{table}[h]
\caption{Metrics  and divergences with their characteristics. $S$ stands for the (power spectrum) density function, $Q$ for the quantile function, and $\text{supp(S)}$ denotes the support of $S(\cdot)$.}
\small
\begin{tabular}{m{2.5cm} m{3.7cm} m{3.5cm} m{2.7cm}}
\toprule
Distance & Definition     & Comments              & Requirements \\ 
\midrule
$L_1$             & $\int_\sR|S(\xi)-S'(\xi)|d\xi$   & Vertical, non-diff., inconclusive if $\text{supp}(S)\neq \text{supp}(S')$  & $\int_\sR|S(\xi)|d\xi<\infty$ \\\hline
$L_2$             & $\int_\sR(S(\xi)-S'(\xi))^2d\xi$ &  Vertical, diff., inconclusive if $\text{supp}(S)\neq \text{supp}(S')$ & $\int_\sR|S(\xi)|^2d\xi<\infty$    \\\hline
$W_1$  &  $\int_0^1 | Q(p)-Q'(p)|d p$     & Horizontal, non-diff.                              &  $\int_\sR S(\xi)d\xi=1$, $\int_\sR| \xi | S(\xi)d\xi<\infty$            \\\hline
$W_2$ &   $\int_0^1(Q(p)-Q'(p))^2d p$      &       Horizontal, non-diff.           &  $\int_\sR S(\xi)d\xi=1$, $\int_\sR | \xi |^2 S(\xi)d\xi<\infty$          \\\hline
Kullback-Liebler  &     $\int_\sR \log\left(\frac{S(\xi)}{S'(\xi)}\right) S(\xi)d\xi$   &   Vertical, non-diff.   & $\text{supp}(S)\subseteq \text{supp}(S')$        \\\hline
Itakura-Saito     &  $\int_\sR\left(\frac{S(\xi)}{S'(\xi)}-\log\frac{S(\xi)}{S'(\xi)}-1\right)d\xi$          &     Vertical, non-diff.   &     $\text{supp}(S) \subseteq \text{supp}(S')$ \\\bottomrule
\end{tabular}
\label{table:metrics}
\end{table}
\fi



%Returning to GPs, recall that PSD and kernels are Fourier pairs and thus their relationship is one-to-one. Furthermore, since zero-mean GPs are uniquely determined by their kernels, any distance (or the weaker notion of divergence) for PSDs can be used to endow the space of GPs with new, alternative, topologies that can be used on learning algorithms. 

%as a criterion to comparing GPs thus endowing the space of GPs . Therefore, our hypothesis is that the \ distance can be a sound alternative to maximum-likelihood training of GPs, since it is i) interpretable as it computes the displacement of energy across the frequency space, and ii) inexpensive to compute as it involves periodograms and one-dimensional Wasserstein distances. 

%In the following, with a slight abuse of notation we will denote the $2$-Wasserstein distance between two measures with probability density functions $f_\mu$ and $f_\nu$ as $W_2(f_\mu,f_\nu)$, and we will refer to it simply as \emph{Wasserstein distance}.


%which, for one-dimensional measures $\mu$ and $\nu$, admits the expression \cite[Theorem 2]{ruschendorf1985wasserstein}
%\begin{equation}
%\label{def:OT}
%W_2(\mu,\nu)=\left(\int_0^1 | Q_{\mu}(p) -Q_{\nu}(p)|^2d p\right)^{1/2},
%\end{equation}
%where $Q_{\mu}(p)$ is the \emph{quantile} function (or generalised inverse of the cumulative distribution function) of $\mu$, and we assumed that $\mu$ and $\nu$ have finite moments of order $2$. 


{}

\subsection{Related work}

\CR{A classic notion of kernel dissimilarity in the machine learning community is that of \emph{kernel alignment}, a concept introduced by \cite{NIPS2001_1f71e393} which measures the agreement between two kernels or a kernel and a task; this method has been mostly applied for kernel selection in SVM-based regression and classification. This notion of dissimilarity is based on the Frobenius inner product between the Gram matrices of each kernel given a dataset---see \citep[Def.~1]{NIPS2001_1f71e393}. Though, in spirit, this concept is related to ours in that the kernel is learnt by minimising a discrepancy measure, we take a signal-processing inspired perspective and exploit the fact that, for stationary GPs, kernels are single-input covariance functions and thus admit computationally-efficient discrepancy measures. In addition to the reference above, the interested reader is referred to \citep{JMLR:v13:cortes12a} for the \emph{centred} kernel alignment method.}

\CR{Within the GP community}, two methodologies for accelerated training can be identified. The first one focuses directly on the  optimisation procedure by, e.g., avoiding inverses~\citep{wilk2020variational}, or derivatives~\citep{rios2018learning}, or even by parallelisation; combining these techniques has allowed to process even a million datapoints~\citep{ke2019exact}. 
%%%%%%%%%%%%%%%
A second perspective is that of sparse GP approximations using \emph{pseudo-inputs}~\citep{quinonero2005unifying}, with particular emphasis on variational methods~\citep{titsias2009variational}. This has allowed for fitting GPs to large datasets~\citep{hensman2013gaussian}, training non-parametric kernels~\citep{tobar2015learning}, and implementing deep GPs~\citep{damianou2013deep,salimbeni2017doubly}. 

 The Wasserstein distance has been used to compare the laws of the GP~\citep{masarotto2019procrustes,mallasto2017learning}, and applied to kernel design, in particular to define GPs~\citep{francois2018gaussian} and deep GPs~\citep{popescu2020hierarchical} over the space of probability distributions.

In geostatistics, the variogram function~\citep{cressie1993stats,chiles1999geo} is defined as the variance of the difference of a process $y$ at two locations $t_1$ and $t_2$, that is, $\gamma(t_1-t_2) = \mathbb{V}[{y(t_1)-y(t_2)}]$. The variogram is computed by choosing a parametric form for $\gamma(t)$ and then fit it to a cloud of points (sample variogram) using least squares. Common variogram functions in the literature include exponential and Gaussian ones, thus drawing a natural connection with GP models. Furthermore, when the process $y$ is stationary and isotropic (or one-dimensional) as in the GP models considered here, the variogram and the covariance $K(t)$ follow the relationship $\gamma(t) = K(0) - K(t)$, therefore, given a kernel function the corresponding variogram function can be clearly identified (and vice versa). The way in which the variogram is fitted in the geostatistics literature is what inspires the methodology proposed here: we fit parametric forms of the covariance (or the PSD) to their corresponding sample approximations in order to find appropriate values for the kernel hyperparameters. Also, as we explore different distances for the covariance and PSD beyond the Euclidean one (least squares) we refer to our proposal as the \emph{Generalised Variogram Method} (GVM).

GVM complements the literature in a way that is orthogonal to the above developments. We find the hyperparameters of a GP in a likelihood-free manner by minimising a loss function operating directly on the sample covariance or its Fourier transform. As we will see, GVM is robust to empirical approximations of the covariance or PSDs, admits arbitrary distances and has a remarkably low computational complexity. %We propose to train GPs by projecting the empirical power spectrum to the space of parametrised spectral densities, which is one-to-one to the space of unit-variance stationary GPs. Furthermore, as the PSDs for unidimensional stationary process are densities supported on $\R$ (and are usually compact), most distances between them are straightforward to compute at a cost that is linear in the frequency grid. Therefore, the proposed method is expected to provide a critical, two-order-of-magnitude, improvement over the vanilla, cubic cost, ML procedure. In this regard, perhaps the work that is closest to our own is that of \cite{WF2021} which introduces the Wasserstein-Fourier distance of general time series, however, they do not consider the use of the metric for learning.  

